Disentangling the independently controllable factors of variation by interacting with the world

It has been postulated that a good representation is one that disentangles the underlying explanatory factors of variation. However, it remains an open question what kind of training framework could potentially achieve that. Whereas most previous work focuses on the static setting (e.g., with images), we postulate that some of the causal factors could be discovered if the learner is allowed to interact with its environment. The agent can experiment with different actions and observe their effects. More specifically, we hypothesize that some of these factors correspond to aspects of the environment which are independently controllable, i.e., that there exists a policy and a learnable feature for each such aspect of the environment, such that this policy can yield changes in that feature with minimal changes to other features that explain the statistical variations in the observed data. We propose a specific objective function to find such factors, and verify experimentally that it can indeed disentangle independently controllable aspects of the environment without any extrinsic reward signal.

==> images/recovering.tex <==
\begin{tikzpicture}
\node[inner sep=0pt] (im0) at (0,0)
    {\fbox{\includegraphics[width=.25\textwidth]{im_causal0_good.png}}};
\node[inner sep=0pt] (im1) at (5,0)
    {\fbox{\includegraphics[width=.25\textwidth]{im_causal1_good.png}}};


\node[] (ht) at (0,-3) {$\underbrace{h_1}_{(0.4,\ 13.1)}$};
\node[] (ht1) at (5,-3) {$\underbrace{h_2}_{(5.9,\ -11.6)}$}; 
\node[] (dh) at (2.5,-5) {$dh ={(5.5,\ -24.8)} \approx 2\cdot dh_{{\color{green} down}} + 3\cdot dh_{{\color{red} right}}$};
    \draw[->,thick] (im0.south) -- (ht.north)
    node[midway,fill=white] {Encoder};
    \draw[<-,thick] (ht1) -- (im1.south)
    node[midway,fill=white] {Encoder};
    
    \draw[->,thick] (ht.east) -- (dh.north);
     \draw[->,thick] (ht1.west) -- (dh.north);
    
\end{tikzpicture}
%  = h + \underbrace{dh_{right}}_{(5,\ -5)} + \underbrace{2\cdot dh_{{\color{green} {\color{green} down}}}}_{(-10,\ -10)}

==> oldbibliography.tex <==
\begin{thebibliography}{28}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{\texttt{#1}}
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi: #1}\else
  \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi

\bibitem[Bacon et~al.(2016)Bacon, Harb, and Precup]{bacon2016option}
Pierre-Luc Bacon, Jean Harb, and Doina Precup.
\newblock {The option-critic architecture}.
\newblock \emph{arXiv preprint arXiv:1609.05140}, 2016.

\bibitem[Bengio(2009)]{Bengio-2009-book}
Yoshua Bengio.
\newblock \emph{Learning deep architectures for {AI}}.
\newblock Now Publishers, 2009.

\bibitem[David~Silver(2017)]{silver2017}
Matteo Hessel Tom Schaul Arthur Guez Tim Harley Gabriel Dulac-Arnold David
  Reichert Neil Rabinowitz Andre Barreto Thomas~Degris David~Silver, Hado
  van~Hasselt.
\newblock {The Predictron: End-To-End Learning and Planning}.
\newblock \emph{arXiv}, \penalty0 (arXiv:1612.08810), 2017.

\bibitem[Dayan(1993)]{dayan1993improving}
Peter Dayan.
\newblock {Improving generalization for temporal difference learning: The
  successor representation}.
\newblock \emph{Neural Computation}, 5\penalty0 (4):\penalty0 613--624, 1993.

\bibitem[Dayan et~al.(1995)Dayan, Hinton, Neal, and Zemel]{Dayan-et-al-1995}
Peter Dayan, Geoffrey~E Hinton, Radford~M Neal, and Richard~S Zemel.
\newblock The {H}elmholtz machine.
\newblock \emph{Neural computation}, 7\penalty0 (5):\penalty0 889--904, 1995.

\bibitem[Dinh et~al.(2014)Dinh, Krueger, and Bengio]{Dinh-et-al-2014}
Laurent Dinh, David Krueger, and Yoshua Bengio.
\newblock {NICE: Non-linear Independent Components Estimation}.
\newblock arXiv:1410.8516, ICLR 2015 workshop, 2014.

\bibitem[Glynn(1987)]{glynn1987likelilood}
Peter~W Glynn.
\newblock {Likelilood ratio gradient estimation: an overview}.
\newblock In \emph{Proceedings of the 19th conference on Winter simulation},
  pages 366--375. ACM, 1987.

\bibitem[Goodfellow et~al.(2016)Goodfellow, Bengio, and
  Courville]{Goodfellow-et-al-2016}
Ian Goodfellow, Yoshua Bengio, and Aaron Courville.
\newblock \emph{Deep Learning}.
\newblock MIT Press, 2016.
\newblock \url{http://www.deeplearningbook.org}.

\bibitem[Goodfellow et~al.(2014)Goodfellow, Pouget-Abadie, Mirza, Xu,
  Warde-Farley, Ozair, Courville, and Bengio]{Goodfellow-et-al-NIPS2014}
Ian~J. Goodfellow, Jean Pouget-Abadie, Mehdi Mirza, Bing Xu, David
  Warde-Farley, Sherjil Ozair, Aaron Courville, and Yoshua Bengio.
\newblock {Generative Adversarial Networks}.
\newblock In \emph{NIPS'2014}, 2014.

\bibitem[Gopnik and Wellman(2012)]{gopnik}
Alison Gopnik and Henry~M. Wellman.
\newblock {Reconstructing constructivism: Causal models, Bayesian learning
  mechanisms and the theory theory}.
\newblock \emph{Psychological Bulletin}, 138\penalty0 (6):\penalty0 1085, 2012.

\bibitem[Greff et~al.(2016)Greff, Rasmus, Berglund, Hao, Valpola, and
  Schmidhuber]{greff2016tagger}
Klaus Greff, Antti Rasmus, Mathias Berglund, Tele Hao, Harri Valpola, and
  Juergen Schmidhuber.
\newblock {Tagger: Deep unsupervised perceptual grouping}.
\newblock In \emph{Advances in Neural Information Processing Systems}, pages
  4484--4492, 2016.

\bibitem[Hinton and Salakhutdinov(2006)]{hinton2006reducing}
Geoffrey~E Hinton and Ruslan~R Salakhutdinov.
\newblock {Reducing the dimensionality of data with neural networks}.
\newblock \emph{Science}, 313\penalty0 (5786):\penalty0 504--507, 2006.

\bibitem[Hyvarinen and Morioka(2016)]{Hyvarinen+Morioka-NIPS2016}
Aapo Hyvarinen and Hiroshi Morioka.
\newblock {Unsupervised Feature Extraction by Time-Contrastive Learning and
  Nonlinear {ICA}}.
\newblock In \emph{NIPS}, 2016.

\bibitem[Ioffe and Szegedy(2015)]{ioffe2015batch}
Sergey Ioffe and Christian Szegedy.
\newblock Batch normalization: Accelerating deep network training by reducing
  internal covariate shift.
\newblock In \emph{International Conference on Machine Learning}, pages
  448--456, 2015.

\bibitem[Jaderberg et~al.(2016)Jaderberg, Mnih, Czarnecki, Schaul, Leibo,
  Silver, and Kavukcuoglu]{jaderberg2016reinforcement}
Max Jaderberg, Volodymyr Mnih, Wojciech~Marian Czarnecki, Tom Schaul, Joel~Z
  Leibo, David Silver, and Koray Kavukcuoglu.
\newblock {Reinforcement learning with unsupervised auxiliary tasks}.
\newblock \emph{arXiv preprint arXiv:1611.05397}, 2016.

\bibitem[Kingma and Ba(2014)]{kingma2014adam}
Diederik Kingma and Jimmy Ba.
\newblock {Adam: A method for stochastic optimization}.
\newblock \emph{arXiv preprint arXiv:1412.6980}, 2014.

\bibitem[Kingma and Welling(2014)]{Kingma+Welling-ICLR2014}
Durk~P. Kingma and Max Welling.
\newblock {Auto-encoding variational Bayes}.
\newblock In \emph{Proceedings of the International Conference on Learning
  Representations (ICLR)}, 2014.

\bibitem[Kulkarni et~al.(2016)Kulkarni, Saeedi, Gautam, and
  Gershman]{kulkarni2016deep}
Tejas~D Kulkarni, Ardavan Saeedi, Simanta Gautam, and Samuel~J Gershman.
\newblock {Deep successor reinforcement learning}.
\newblock \emph{arXiv preprint arXiv:1606.02396}, 2016.

\bibitem[LeCun(1998)]{lecun1998mnist}
Yann LeCun.
\newblock {The MNIST database of handwritten digits}.
\newblock \emph{http://yann.lecun.com/exdb/mnist/}, 1998.

\bibitem[Minin et~al.(2012)Minin, Knoll, Zimmermann, Siemens, and
  Siemens]{minin2012complex}
Alexey Minin, Alois Knoll, Hans-Georg Zimmermann, AG~Siemens, and LLC Siemens.
\newblock {Complex Valued Artificial Recurrent Neural Network as a Novel
  Approach to Model the Perceptual Binding Problem.}
\newblock In \emph{ESANN}. Citeseer, 2012.

\bibitem[Oh et~al.(2015)Oh, Guo, Lee, Lewis, and Singh]{oh2015action}
Junhyuk Oh, Xiaoxiao Guo, Honglak Lee, Richard~L Lewis, and Satinder Singh.
\newblock {Action-conditional video prediction using deep networks in atari
  games}.
\newblock In \emph{Advances in Neural Information Processing Systems}, pages
  2863--2871, 2015.

\bibitem[Precup(2000)]{precup2000temporal}
Doina Precup.
\newblock {Temporal abstraction in reinforcement learning}.
\newblock 2000.

\bibitem[Ratitch and Precup(2003)]{ratitch}
Bohdana Ratitch and Doina Precup.
\newblock {Using MDP Characteristics to Guide Exploration in Reinforcement
  Learning}.
\newblock In \emph{ECML}, pages 313--324, 2003.

\bibitem[Sukhbaatar et~al.(2015)Sukhbaatar, Szlam, Synnaeve, Chintala, and
  Fergus]{sukhbaatar2015mazebase}
Sainbayar Sukhbaatar, Arthur Szlam, Gabriel Synnaeve, Soumith Chintala, and Rob
  Fergus.
\newblock {MazeBase: A sandbox for learning from games}.
\newblock \emph{arXiv preprint arXiv:1511.07401}, 2015.

\bibitem[Sutton(2011)]{sutton2009}
Modayil J. Delp M. Degris T. Pilarski P. M. White A. Precup-D. Sutton, R.~S.
\newblock {Horde: A scalable real-time architecture for learning knowledge from
  unsupervised sensorimotor interaction}.
\newblock In \emph{AAMAS}, 2011.

\bibitem[Sutton et~al.(1999)Sutton, Precup, and Singh]{sutton1999between}
Richard~S Sutton, Doina Precup, and Satinder Singh.
\newblock {Between MDPs and semi-MDPs: A framework for temporal abstraction in
  reinforcement learning}.
\newblock \emph{Artificial intelligence}, 112\penalty0 (1-2):\penalty0
  181--211, 1999.

\bibitem[Vincent et~al.(2008)Vincent, Larochelle, Bengio, and
  Manzagol]{VincentICML2008}
Pascal Vincent, Hugo Larochelle, Yoshua Bengio, and Pierre-Antoine Manzagol.
\newblock Extracting and composing robust features with denoising autoencoders.
\newblock In \emph{ICML 2008}, 2008.

\bibitem[Williams(1992)]{williams1992simple}
Ronald~J Williams.
\newblock {Simple statistical gradient-following algorithms for connectionist
  reinforcement learning}.
\newblock \emph{Machine learning}, 8\penalty0 (3-4):\penalty0 229--256, 1992.

\end{thebibliography}
